Fine-grained Manipulation Attacks to Local Differential Privacy Protocols for Data Streams

Local Differential Privacy (LDP) enables massive data collection and analysis while protecting end users' privacy against untrusted aggregators. It has been applied to various data types (e.g., categorical, numerical, and graph data) and application settings (e.g., static and streaming). Recent findings indicate that LDP protocols can be easily disrupted by poisoning or manipulation attacks, which leverage injected/corrupted fake users to send crafted data conforming to the LDP reports. However, current attacks primarily target static protocols, neglecting the security of LDP protocols in the streaming settings. Our research fills the gap by developing novel fine-grained manipulation attacks to LDP protocols for data streams. By reviewing the attack surfaces in existing algorithms, We introduce a unified attack framework with composable modules, which can manipulate the LDP estimated stream toward a target stream. Our attack framework can adapt to state-of-the-art streaming LDP algorithms with different analytic tasks (e.g., frequency and mean) and LDP models (event-level, user-level, w-event level). We validate our attacks theoretically and through extensive experiments on real-world datasets, and finally explore a possible defense mechanism for mitigating these attacks.

==> Reference.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{duchi2013local}
J.~Duchi, M.~Jordan, and M.~Wainwright, ``Local privacy and statistical minimax rates,'' in \emph{Proc. IEEE FOCS}, 2013, pp. 429--438.

\bibitem{duchi2014privacy}
------, ``Privacy aware learning,'' \emph{Journal of the ACM (JACM)}, vol.~61, no.~6, pp. 1--57, 2014.

\bibitem{kasiviswanathan2011can}
S.~Kasiviswanathan, H.~Lee, N, S.~Raskhodnikova, and A.~Smith, ``What can we learn privately?'' \emph{SIAM J. Computing}, vol.~40, no.~3, pp. 793--826, 2011.

\bibitem{Erlingsson2014RAPPORRA}
{\'U}.~Erlingsson, A.~Korolova, and V.~Pihur, ``Rappor: Randomized aggregatable privacy-preserving ordinal response,'' in \emph{Proc. ACM CCS}, 2014, pp. 1054--1067.

\bibitem{ding2017collecting}
B.~Ding, J.~Kulkarni, and S.~Yekhanin, ``Collecting telemetry data privately,'' in \emph{Proc. NeurIPS}, 2017, pp. 3574--3583.

\bibitem{AppleDP}
\BIBentryALTinterwordspacing
differential privacy team~at Apple, ``Learning with privacy at scale,'' 2017. [Online]. Available: \url{https://machinelearning.apple.com/research/learning-with-privacy-at-scale}
\BIBentrySTDinterwordspacing

\bibitem{arcolezi2021random}
H.~Arcolezi, J.~Couchot, B.~Al~Bouna, and X.~Xiao, ``Random sampling plus fake data: Multidimensional frequency estimates with local differential privacy,'' in \emph{Proc. of ACM CIKM}, 2021, pp. 47--57.

\bibitem{kairouz2016extremal}
P.~Kairouz, S.~Oh, and P.~Viswanath, ``Extremal mechanisms for local differential privacy,'' \emph{J. Mach. Learn. Res.}, vol.~17, no.~1, pp. 492--542, 2016.

\bibitem{Wang2017LocallyDPFE}
T.~Wang, J.~Blocki, N.~Li, and S.~Jha, ``Locally differentially private protocols for frequency estimation,'' in \emph{Proc. USENIX Security}, 2017, pp. 729--745.

\bibitem{arcolezi2022frequency}
H.~H. Arcolezi, C.~Pinz{\'o}n, C.~Palamidessi, and S.~Gambs, ``Frequency estimation of evolving data under local differential privacy,'' \emph{arXiv preprint arXiv:2210.00262}, 2022.

\bibitem{arcolezi2022improving}
H.~H. Arcolezi, J.-F. Couchot, B.~Bouna, and X.~Xiao, ``Improving the utility of locally differentially private protocols for longitudinal and multidimensional frequency estimates. digital communications and networks (2022),'' 2022.

\bibitem{ohrimenko2022randomize}
O.~Ohrimenko, A.~Wirth, and H.~Wu, ``Randomize the future: Asymptotically optimal locally private frequency estimation protocol for longitudinal data,'' in \emph{Proceedings of the 41st ACM SIGMOD-SIGACT-SIGAI Symposium on Principles of Database Systems}, 2022, pp. 237--249.

\bibitem{Wang2019CollectingAA}
N.~Wang, X.~Xiao, Y.~Yang, J.~Zhao, S.~Hui, H.~Shin, J.~Shin, and G.~Yu, ``Collecting and analyzing multidimensional data with local differential privacy,'' in \emph{Proc. IEEE ICDE}, 2019, pp. 638--649.

\bibitem{ye2019privkv}
Q.~Ye, H.~Hu, X.~Meng, and H.~Zheng, ``Privkv: Key-value data collection with local differential privacy,'' in \emph{Proc. IEEE SP}, 2019, pp. 317--331.

\bibitem{Qin2016HeavyHE}
Z.~Qin, Y.~Yang, T.~Yu, I.~Khalil, X.~Xiao, and K.~Ren, ``Heavy hitter estimation over set-valued data with local differential privacy,'' in \emph{Proc. ACM CCS}, 2016, pp. 192--203.

\bibitem{li2022frequent}
J.~Li, W.~Gan, Y.~Gui, Y.~Wu, and P.~S. Yu, ``Frequent itemset mining with local differential privacy,'' in \emph{Proceedings of the 31st ACM International Conference on Information \& Knowledge Management}, 2022, pp. 1146--1155.

\bibitem{wang2018privset}
S.~Wang, L.~Huang, Y.~Nie, P.~Wang, H.~Xu, and W.~Yang, ``Privset: Set-valued data analyses with locale differential privacy,'' in \emph{IEEE INFOCOM 2018-IEEE Conference on Computer Communications}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2018, pp. 1088--1096.

\bibitem{wang2018locally}
T.~Wang, N.~Li, and S.~Jha, ``Locally differentially private frequent itemset mining,'' in \emph{2018 IEEE Symposium on Security and Privacy (SP)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2018, pp. 127--143.

\bibitem{Imola2021LDPgraph}
J.~Imola, T.~Murakami, and K.~Chaudhuri, ``Locally differentially private analysis of graph statistics,'' in \emph{30th USENIX security symposium (USENIX Security 21)}, 2021, pp. 983--1000.

\bibitem{Ye2020LDPgraph}
Q.~Ye, H.~Hu, M.~H. Au, X.~Meng, and X.~Xiao, ``Towards locally differentially private generic graph metric estimation,'' in \emph{2020 IEEE 36th International Conference on Data Engineering (ICDE)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2020, pp. 1922--1925.

\bibitem{wang2020continuous}
T.~Wang, J.-Q. Chen, Z.~Zhang, D.~Su, Y.~Cheng, Z.~Li, N.~Li, and S.~Jha, ``Continuous release of data streams under both centralized and local differential privacy,'' in \emph{Proc. ACM CCS}, 2021, pp. 1237--1253.

\bibitem{baocgm}
E.~Bao, Y.~Yang, X.~Xiao, and B.~Ding, ``Cgm: An enhanced mechanism for streaming data collection with local differential privacy,'' \emph{Proc. of VLDB Endow.}, vol.~14, no.~11, pp. 2258--2270, 2021.

\bibitem{LDP_IDS}
X.~Ren, L.~Shi, W.~Yu, S.~Yang, C.~Zhao, and Z.~Xu, ``Ldp-ids: Local differential privacy for infinite data streams,'' in \emph{Proceedings of the 2022 international conference on management of data}, 2022, pp. 1064--1077.

\bibitem{schaler2023benchmarking}
C.~Sch{\"a}ler, T.~H{\"u}tter, and M.~Sch{\"a}ler, ``Benchmarking the utility of w-event differential privacy mechanisms-when baselines become mighty competitors,'' \emph{Proceedings of the VLDB Endowment}, vol.~16, no.~8, pp. 1830--1842, 2023.

\bibitem{li2023privsketch}
Y.~Li, X.~Lee, B.~Peng, T.~Palpanas, and J.~Xue, ``Privsketch: A private sketch-based frequency estimation protocol for data streams,'' \emph{arXiv preprint arXiv:2306.12144}, 2023.

\bibitem{joseph2018local}
M.~Joseph, A.~Roth, J.~Ullman, and B.~Waggoner, ``Local differential privacy for evolving data,'' \emph{Proc. NeurIPS}, vol.~31, pp. 2375--2384, 2018.

\bibitem{Erlingsson2019AmplificationBS}
{\'U}.~Erlingsson, V.~Feldman, I.~Mironov, A.~Raghunathan, K.~Talwar, and A.~Thakurta, ``Amplification by shuffling: From local to central differential privacy via anonymity,'' \emph{ArXiv}, vol. abs/1811.12469, 2019.

\bibitem{10.1145/3639292}
\BIBentryALTinterwordspacing
J.~Zhang, C.~Zhang, G.~Li, and C.~Chai, ``Pace: Poisoning attacks on learned cardinality estimation,'' \emph{Proc. ACM Manag. Data}, vol.~2, no.~1, Mar. 2024. [Online]. Available: \url{https://doi.org/10.1145/3639292}
\BIBentrySTDinterwordspacing

\bibitem{10.1145/3514221.3517867}
\BIBentryALTinterwordspacing
E.~M. Kornaropoulos, S.~Ren, and R.~Tamassia, ``The price of tailoring the index to your data: Poisoning attacks on learned index structures,'' in \emph{Proceedings of the 2022 International Conference on Management of Data}, ser. SIGMOD '22.\hskip 1em plus 0.5em minus 0.4em\relax New York, NY, USA: Association for Computing Machinery, 2022, p. 1331–1344. [Online]. Available: \url{https://doi.org/10.1145/3514221.3517867}
\BIBentrySTDinterwordspacing

\bibitem{Cao2021poisonFE}
X.~Cao, J.~Jia, and N.~Z. Gong, ``Data poisoning attacks to local differential privacy protocols,'' in \emph{30th USENIX Security Symposium (USENIX Security 21)}, 2021, pp. 947--964.

\bibitem{Wu2022poisonKey}
Y.~Wu, X.~Cao, J.~Jia, and N.~Z. Gong, ``Poisoning attacks to local differential privacy protocols for $\{$Key-Value$\}$ data,'' in \emph{31st USENIX Security Symposium (USENIX Security 22)}, 2022, pp. 519--536.

\bibitem{Li2023Finegrained}
X.~Li, N.~Li, W.~Sun, N.~Z. Gong, and H.~Li, ``Fine-grained poisoning attack to local differential privacy protocols for mean and variance estimation,'' in \emph{32nd USENIX Security Symposium (USENIX Security 23)}, 2023, pp. 1739--1756.

\bibitem{Kellaris2014DifferentiallyPE}
G.~Kellaris, S.~Papadopoulos, X.~Xiao, and D.~Papadias, ``Differentially private event sequences over infinite streams,'' \emph{Proc. VLDB Endow.}, vol.~7, pp. 1155--1166, 2014.

\bibitem{ZhangWLHC18}
Z.~Zhang, T.~Wang, N.~Li, S.~He, and J.~Chen, ``Calm: Consistent adaptive local marginal for marginal release under local differential privacy,'' in \emph{Proc. ACM CCS}, 2018, pp. 212--229.

\bibitem{Duchi2016MinimaxOP}
J.~Duchi, M.~Wainwright, and M.~Jordan, ``Minimax optimal procedures for locally private estimation,'' \emph{J. Am. Stat. Assoc}, vol. 113, pp. 182 -- 201, 2016.

\bibitem{Wang2016RescueDPRS}
Q.~Wang, Y.~Zhang, X.~Lu, Z.~Wang, Z.~Qin, and K.~Ren, ``Rescuedp: Real-time spatio-temporal crowd-sourced data publishing with differential privacy,'' \emph{Proc. IEEE INFOCOM}, pp. 1--9, 2016.

\bibitem{10.1145/2806416.2806441}
H.~Li, L.~Xiong, X.~Jiang, and J.~Liu, ``Differentially private histogram publication for dynamic datasets: An adaptive sampling approach,'' in \emph{Proc. of ACM CIKM}, 2015, p. 1001–1010.

\bibitem{Chen2017PeGaSusDD}
Y.~Chen, A.~Machanavajjhala, M.~Hay, and G.~Miklau, ``Pegasus: Data-adaptive differentially private stream processing,'' \emph{Proc. ACM CCS}, pp. 1375--1388, 2017.

\bibitem{Fan2014AnAA}
L.~Fan and L.~Xiong, ``An adaptive approach to real-time aggregate monitoring with differential privacy,'' \emph{IEEE Trans. on Knowl. Data Eng.}, vol.~26, pp. 2094--2106, 2014.

\bibitem{thomas2013trafficking}
K.~Thomas, D.~McCoy, C.~Grier, A.~Kolcz, and V.~Paxson, ``$\{$Trafficking$\}$ fraudulent accounts: The role of the underground market in twitter spam and abuse,'' in \emph{22nd USENIX Security Symposium (USENIX Security 13)}, 2013, pp. 195--210.

\bibitem{tong2024data}
W.~Tong, H.~Chen, J.~Niu, and S.~Zhong, ``Data poisoning attacks to locally differentially private frequent itemset mining protocols,'' in \emph{Proc. ACM CCS}, 2024.

\bibitem{huangfu2018parallelizing}
Q.~Huangfu and J.~J. Hall, ``Parallelizing the dual revised simplex method,'' \emph{Mathematical Programming Computation}, vol.~10, no.~1, pp. 119--142, 2018.

\bibitem{Cao2021Provably}
X.~Cao, J.~Jia, and N.~Z. Gong, ``Provably secure federated learning against malicious clients,'' in \emph{Proceedings of the AAAI conference on artificial intelligence}, vol.~35, no.~8, 2021, pp. 6885--6893.

\bibitem{Liu2008IsolationForest}
F.~T. Liu, K.~M. Ting, and Z.-H. Zhou, ``Isolation forest,'' in \emph{2008 eighth ieee international conference on data mining}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2008, pp. 413--422.

\bibitem{Dwork2014TheAF}
C.~Dwork and A.~Roth, ``The algorithmic foundations of differential privacy,'' \emph{Found. Trends Theor. Comput. Sci.}, vol.~9, pp. 211--407, 2014.

\bibitem{Dwork-405}
C.~Dwork, ``Differential privacy,'' in \emph{Proc. ICALP}, 2006, pp. 1--12.

\bibitem{xue2022ddrm}
Q.~Xue, Q.~Ye, H.~Hu, Y.~Zhu, and J.~Wang, ``Ddrm: A continual frequency estimation mechanism with local differential privacy,'' \emph{IEEE Transactions on Knowledge and Data Engineering}, 2022.

\bibitem{li2023locally}
X.~Li, Y.~Cao, and M.~Yoshikawa, ``Locally private streaming data release with shuffling and subsampling,'' in \emph{2023 IEEE 39th International Conference on Data Engineering Workshops (ICDEW)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2023, pp. 125--131.

\bibitem{gao2023privacy}
W.~Gao and S.~Zhou, ``Privacy-preserving for dynamic real-time published data streams based on local differential privacy,'' \emph{IEEE Internet of Things Journal}, 2023.

\bibitem{ye2021beyond}
Q.~Ye, H.~Hu, N.~Li, X.~Meng, H.~Zheng, and H.~Yan, ``Beyond value perturbation: Local differential privacy in the temporal setting,'' in \emph{IEEE INFOCOM 2021-IEEE Conference on Computer Communications}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2021, pp. 1--10.

\bibitem{10.1145/1806689.1806787}
C.~Dwork, M.~Naor, T.~Pitassi, and G.~N. Rothblum, ``Differential privacy under continual observation,'' in \emph{Proc. ACM STOC}, 2010, pp. 715--724.

\bibitem{cheu2021manipulation}
A.~Cheu, A.~Smith, and J.~Ullman, ``Manipulation attacks in local differential privacy,'' in \emph{2021 IEEE Symposium on Security and Privacy (SP)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2021, pp. 883--900.

\bibitem{zheng2024data}
Z.~Zheng, Z.~Li, C.~Huang, S.~Long, M.~Li, and X.~Shen, ``Data poisoning attacks and defenses to ldp-based privacy-preserving crowdsensing,'' \emph{IEEE Transactions on Dependable and Secure Computing}, 2024.

\bibitem{li2020estimating}
Z.~Li, T.~Wang, M.~Lopuha{\"a}-Zwakenberg, N.~Li, and B.~{\v{S}}koric, ``Estimating numerical distributions under local differential privacy,'' in \emph{Proc. ACM SIGMOD}, 2020, pp. 621--635.

\end{thebibliography}

